Is Free Self-Alignment Possible?

Aligning pretrained language models (LMs) often requires large-scale preference data and substantial computational resources. These costs become even more prohibitive for multi-objective or pluralistic alignment. Is this truly necessary? Can we perform efficient alignment using only internal model capabilities, and without additional training? To answer this question, we propose AlignEZ, a novel approach that leverages (1) self-generated preference data and (2) representation editing to achieve cost-effective, efficient alignment. By operating directly on learned representations, AlignEZ independently targets different behavioral aspects without the overhead of traditional alignment methods. Our experiments reveal that this cost-efficient procedure improves performance across diverse tasks: up to 19.9% on general alignment and 1.9% on challenging mathematical reasoning tasks, even when starting from a strong base model. AlignEZ can also align models to multiple objectives simultaneously, granting fine-grained control over multiple preference axes. Finally, we show that AlignEZ can accelerate more expensive alignment procedures--such as DPO--even under limited availability of ground-truth preference data.

==> figs/main_exp_plots.tex <==
\begin{figure}[t!]

\centering

\includegraphics[width=0.48\textwidth]{figs/main_plots/Engagement.png}%
\hspace{1.3em}
\includegraphics[width=0.48\textwidth]{figs/main_plots/Helpfulness.png}%
\\
% \vspace{1em}
\includegraphics[width=0.48\textwidth]{figs/main_plots/Depth.png}%
\hspace{1.3em}
\includegraphics[width=0.48\textwidth]{figs/main_plots/Factuality.png}%
\\
% \vspace{1em}
\includegraphics[width=0.48\textwidth]{figs/main_plots/Clarity.png}%
\hspace{1.3em}
\includegraphics[width=0.48\textwidth]{figs/main_plots/Average.png}%

\caption{$\SYSNAME$ \textbf{Relative Improvement\%}. The y-axis shows the Relative Improvement\%: how much $\SYSNAME$ enhances the base model's performance compared to an aligned version. Values are recorded across six datasets (x-axis). A value of 100\% means $\SYSNAME$ improves the base model to the same extent as the aligned version, while 0\% means $\SYSNAME$ performs the same as the base model. Performance is recorded for three model families: Mistral (orange), Llama2 (green), and Llama3 (blue). We observe substantial improvements in the base models, resulting in a narrower performance gap between the base models and the aligned versions.}
\label{fig:main_exp}

\end{figure}

==> figs/micro_logreg.tex <==
\begin{figure}[]\centering
\subfloat{\label{a}\includegraphics[width=.25\linewidth]{figs/micro_logreg/mistral.png}}
% \hfill
\subfloat{\label{b}\includegraphics[width=.25\linewidth]{figs/micro_logreg/llama2.png}}
% \hfill
% \vspace{-1.5em}
\subfloat{\label{c}\includegraphics[width=.25\linewidth]{figs/micro_logreg/Llama3.png}}
\caption{Net win\% (blue, top row) correlation with self-generated data quality (orange, bottom row). Left to right: Mistral, Llama2, Llama3.}
\label{fig:micro}
\end{figure}

==> figs/motivating_exp.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{ICLR 2025 Template/figs/time_sensitive_exp.png}
    \caption{Motivating experiment. Expensive alignment techniques like DPO is unreliable in low-data regime}
    \label{fig:enter-label}
\end{figure}

==> figs/single_multiobj.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/single_llama32.pdf}
    \caption{Single direction steering}
    \label{fig:single_llama32}
\end{figure*}

==> tables/dpo_result.tex <==
% % % \begin{figure}
% % % \centering
% % % \includegraphics[width=.5\textwidth]{ICLR 2025 Template/figs/DPO.png}
% % % \caption{$\SYSNAME$ expedites DPO alignment. DPO with only 1\% data + $\SYSNAME$ matches the performance of DPO with 25\% data (blue dashed line).}\label{fig:dpo}
% % % \end{figure}

% %  % \caption{$\SYSNAME$ expedites DPO alignment. DPO with only 1\% data + $\SYSNAME$ matches the performance of DPO with 25\% data.}\label{fig:dpo}%


% %  \begin{figure}
% % \begin{floatrow}
% % \capbtabbox{%
% %  \small
%  \begin{tabular}{llcc}
%      \toprule
%     Model & Dataset & \textbf{$\Delta\%$} \\
%     \toprule
%      \multirow{3}{*}{Mistral-7B-v0.3} & koala & 9.21 \\
%        & oasst & 6.00 \\
%        & selfinstruct & 3.54  \\
    
%     \midrule

%      \multirow{3}{*}{Llama-3.1-8B } & koala & 10.00 \\
%        & oasst & 10.00  \\
%        & selfinstruct & 5.31  \\
       
%       \bottomrule
% \end{tabular}

% % }{%
% %   \caption{Compatibility with prompting-based methods. $\SYSNAME$ combined with URIAL yields improvements over using URIAL alone.} \label{tab:urial}%
% % }
% % \ffigbox{%
% %   \includegraphics[width=.35\textwidth]{figs/DPO.png}
% % }{%
% %   \caption{DPO with 1\% data + $\SYSNAME$ matches the performance of DPO with 25\% data (blue dashed line). \textcolor{blue}{DPO training and evaluation are done with the UltraFeedback-binarized dataset.}}\label{fig:dpo}%
% % }
% % \end{floatrow}
% % \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/DPO.png}
%     \caption{DPO with 1\% data + $\SYSNAME$ matches the performance of DPO with 25\% data (blue dashed line). \textcolor{blue}{DPO training and evaluation are done with the UltraFeedback-binarized dataset.}
%     \label{fig:dpo}
% \end{figure}

==> tables/main_algorithm.tex <==
\begin{figure}
\begin{algorithm}[H]
        \caption{\textsc{$\SYSNAME$} harmful and helpful subspaces identification} \label{tab:algorithm}
	\begin{algorithmic}[1]
		\STATE \textbf{Parameters:} base pretrained LM $\omega$ with $L$ layers, self-generated preference pairs $P^{help}, P^{harm}$, query $q$
            
            \FOR{$l \in 1,2,\ldots, L$}
                \FOR{$p_i^{help}, p_i^{harm} \in P^{help}, P^{harm}$}
                
                \STATE Get representations $\Phi_{i,l}^{help}, \Phi_{i,l}^{harm}$ from prompts $p^{help}_i, p^{harm}_i$
                \ENDFOR

                
                \STATE Let $K$ be the total number of preference pairs $|P^{help}|$ 
                \STATE Stack embedding matrix $\textbf{H}_l^{help}=\left [\Phi_{1,l}^{help} \middle| \ldots \middle| \Phi_{K,l}^{help}\right ]^T$,
                $\textbf{H}_l^{harm}=\left [\Phi_{1,l}^{harm} \middle| \ldots \middle| \Phi_{K,l}^{harm}\right ]^T$

                \STATE Find k-nearest neighbors of query $q$, $k\text{-NN}(q)$
                % \STATE Index $\textbf{H}_l^{help}$ and $\textbf{H}_l^{harm}$ by the neighbors indexes
                \STATE Identify $\theta_l^{help}$ and  $\theta_l^{harm}$ with Equation \ref{eq:svd} using the embeddings of self-generated preference data associated with k-nearest neighbors
            \ENDFOR
            \STATE \textbf{Returns:} Helpful and harmful subspaces $\theta_l^{help}$, $\theta_l^{harm}$
	\end{algorithmic} 
\end{algorithm}
% \vspace{-5mm}
\end{figure}

==> tables/main_table.tex <==
\begin{table*}
\small
\caption{$\SYSNAME$ significantly improves the base model's performance, closing the gap with aligned models (RLHF and instruction-tuned). Additionally, $\SYSNAME$ consistently outperforms other test-time alignment methods.}
   \label{tab:exp_main}
   \centering
   \setlength\tabcolsep{3.5pt} 
   \begin{tabular}{llcccc|cccc|ccccc}
     \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{Task} &   \multicolumn{4}{c}{ITI + Ground Truth} &  \multicolumn{4}{c}{CAA + Ground Truth} &   \multicolumn{4}{c}{\textbf{$\SYSNAME$}} &  \\ 
    
      \cmidrule(lr){3-6} \cmidrule(lr){7-10}  \cmidrule(lr){11-14}  &  & W\% & L\% & $\Delta\%$ & \textbf{RI} & W\% & L\% & $\Delta\%$ & \textbf{RI} & W\% & L\% & $\Delta\%$ & \textbf{RI} \\
      
    \toprule
     \multirow{5}{*}{Mistral-7B-v0.3}
     & oasst & 28.0 & 33.0 & \cellcolor{blue!10}{-5.0} & \cellcolor{green!10}{-} & 16.0 & 18.0 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-} & 48.0 & 21.0 & \cellcolor{blue!10}{\textbf{27.0}} & \cellcolor{green!10}{\textbf{49.1}} \\
     
     & MT & 11.3  & 28.8 & \cellcolor{blue!10}{-17.5} & \cellcolor{green!10}{-} & 16.25 & 11.25 & \cellcolor{blue!10}{5.0} & \cellcolor{green!10}{\textbf{12.0}} & 32.5 & 35.0 & \cellcolor{blue!10}{-2.5} & \cellcolor{green!10}{-} \\
     
     & helpful-base & 32.7 & 37.6 & \cellcolor{blue!10}{-4.9} & \cellcolor{green!10}{-}  & 15.8 & 10.9 & \cellcolor{blue!10}{5.0} & \cellcolor{green!10}{15.0} & 43.6 & 30.7 & \cellcolor{blue!10}{\textbf{12.9}} & \cellcolor{green!10}{\textbf{38.2}} \\
     
     & self-instruct & 20.4 & 34.5 & \cellcolor{blue!10}{-14.2} & \cellcolor{green!10}{-} & 10 & 12.4 & \cellcolor{blue!10}{-3} & \cellcolor{green!10}{-} & 40.7 & 27.4 & \cellcolor{blue!10}{\textbf{13.3}} & \cellcolor{green!10}{\textbf{27.0}} \\
     
     & koala & 23.7 & 36.8 & \cellcolor{blue!10}{-13.2} & \cellcolor{green!10}{-} & 15.8 & 14.5 & \cellcolor{blue!10}{1.3} & \cellcolor{green!10}{3.0} & 50.0 & 29.0 & \cellcolor{blue!10}{\underline{21.1}} & \cellcolor{green!10}{\underline{43.0}} \\
     
     \midrule

     \multirow{5}{*}{Llama-3.1-8B}
     & oasst & 45.0 & 47.0 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-}  & 47.0 & 33.0 & \cellcolor{blue!10}{4.0} & \cellcolor{green!10}{\underline{100}} & 44.0 & 40.0 & \cellcolor{blue!10}{\textbf{4.0}} & \cellcolor{green!10}{\underline{100}} \\
     
     & MT & 43.0 & 45.6 & \cellcolor{blue!10}{-2.5} & \cellcolor{green!10}{-} & 40.5 & 46.8 & \cellcolor{blue!10}{-6.3} & \cellcolor{green!10}{-} & 41.8 & 39.2 & \cellcolor{blue!10}{\textbf{2.5}} & \cellcolor{green!10}{8.9} \\
     
     & helpful-base & 42.6 & 44.6 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-} & 44.6 & 52.5 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-} & 40.6 & 30.7 & \cellcolor{blue!10}{\textbf{9.9}} & \cellcolor{green!10}{\textbf{9.9}} \\
     
     & self-instruct & 48.7 & 44.3 & \cellcolor{blue!10}{4.4} & \cellcolor{green!10}{\underline{14.7}} & 54.0 & 41.6 & \cellcolor{blue!10}{12.4} & \cellcolor{green!10}{30.1} & 44.3 & 39.8 & \cellcolor{blue!10}{4.4} & \cellcolor{green!10}{\underline{14.7}} \\
     
     & koala & 63.2 & 31.6 & \cellcolor{blue!10}{31.6} & \cellcolor{green!10}{\textbf{100}} & 44.7 & 50.0 & \cellcolor{blue!10}{-5.3} & \cellcolor{green!10}{-} & 42.1 & 53.6 & \cellcolor{blue!10}{-10.5} & \cellcolor{green!10}{-} \\

    
    \bottomrule
   \end{tabular}
 \end{table*}

==> tables/personalization.tex <==

\begin{table}[t!]
\small
\caption{Personalization application}
   \label{tab:exp_main}
   \centering
   \setlength\tabcolsep{3.5pt} 
   \begin{tabular}{llcccc|cccc|ccccc}
     \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{Dataset} &   \multicolumn{4}{c}{ITI + Ground Truth} &  \multicolumn{4}{c}{CAA + Ground Truth} &   \multicolumn{4}{c}{\textbf{$\SYSNAME$}} &  \\ 
    
      \cmidrule(lr){3-6} \cmidrule(lr){7-10}  \cmidrule(lr){11-14}  &  & W\% & L\% & $\Delta\%$ & \textbf{RI} & W\% & L\% & $\Delta\%$ & \textbf{RI} & W\% & L\% & $\Delta\%$ & \textbf{RI} \\
      
    \toprule
     \multirow{5}{*}{Mistral-7B-v0.3}
     & oasst & 28.0 & 33.0 & \cellcolor{blue!10}{-5.0} & \cellcolor{green!10}{-} & 16.0 & 18.0 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-} & 48.0 & 21.0 & \cellcolor{blue!10}{\textbf{27.0}} & \cellcolor{green!10}{\textbf{49.1}} \\
     
     & MT & 11.3  & 28.8 & \cellcolor{blue!10}{-17.5} & \cellcolor{green!10}{-} & 16.25 & 11.25 & \cellcolor{blue!10}{5.0} & \cellcolor{green!10}{\textbf{12.0}} & 32.5 & 35.0 & \cellcolor{blue!10}{-2.5} & \cellcolor{green!10}{-} \\
     
     & helpful-base & 32.7 & 37.6 & \cellcolor{blue!10}{-4.9} & \cellcolor{green!10}{-}  & 15.8 & 10.9 & \cellcolor{blue!10}{5.0} & \cellcolor{green!10}{15.0} & 43.6 & 30.7 & \cellcolor{blue!10}{\textbf{12.9}} & \cellcolor{green!10}{\textbf{38.2}} \\
     
     & self-instruct & 20.4 & 34.5 & \cellcolor{blue!10}{-14.2} & \cellcolor{green!10}{-} & 10 & 12.4 & \cellcolor{blue!10}{-3} & \cellcolor{green!10}{-} & 40.7 & 27.4 & \cellcolor{blue!10}{\textbf{13.3}} & \cellcolor{green!10}{\textbf{27.0}} \\
     
     & koala & 23.7 & 36.8 & \cellcolor{blue!10}{-13.2} & \cellcolor{green!10}{-} & 15.8 & 14.5 & \cellcolor{blue!10}{1.3} & \cellcolor{green!10}{3.0} & 50.0 & 29.0 & \cellcolor{blue!10}{\underline{21.1}} & \cellcolor{green!10}{\underline{43.0}} \\
     
     \midrule

     \multirow{5}{*}{Flan-T5 XXL}
     & oasst & 45.0 & 47.0 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-}  & 47.0 & 33.0 & \cellcolor{blue!10}{4.0} & \cellcolor{green!10}{\underline{100}} & 44.0 & 40.0 & \cellcolor{blue!10}{\textbf{4.0}} & \cellcolor{green!10}{\underline{100}} \\
     
     & MT & 43.0 & 45.6 & \cellcolor{blue!10}{-2.5} & \cellcolor{green!10}{-} & 40.5 & 46.8 & \cellcolor{blue!10}{-6.3} & \cellcolor{green!10}{-} & 41.8 & 39.2 & \cellcolor{blue!10}{\textbf{2.5}} & \cellcolor{green!10}{8.9} \\
     
     & helpful-base & 42.6 & 44.6 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-} & 44.6 & 52.5 & \cellcolor{blue!10}{-2.0} & \cellcolor{green!10}{-} & 40.6 & 30.7 & \cellcolor{blue!10}{\textbf{9.9}} & \cellcolor{green!10}{\textbf{9.9}} \\
     
     & self-instruct & 48.7 & 44.3 & \cellcolor{blue!10}{4.4} & \cellcolor{green!10}{\underline{14.7}} & 54.0 & 41.6 & \cellcolor{blue!10}{12.4} & \cellcolor{green!10}{30.1} & 44.3 & 39.8 & \cellcolor{blue!10}{4.4} & \cellcolor{green!10}{\underline{14.7}} \\
     
     & koala & 63.2 & 31.6 & \cellcolor{blue!10}{31.6} & \cellcolor{green!10}{\textbf{100}} & 44.7 & 50.0 & \cellcolor{blue!10}{-5.3} & \cellcolor{green!10}{-} & 42.1 & 53.6 & \cellcolor{blue!10}{-10.5} & \cellcolor{green!10}{-} \\

    
    \bottomrule
   \end{tabular}
 \end{table}

==> tables/subspace_correlations.tex <==
 \begin{table}
 \centering
 \begin{tabular}{llc|c}
 
     \toprule
    Preference Pair  & Avg. Cosine Sim  \\
    \toprule
    Helpful, Harmless & 0.246 \\
    \midrule
    Helpful, Humor & -0.184 \\
    \midrule
    Harmless, Humor & -0.199 \\
    \bottomrule
\caption{Preference pair correlation. We measure the cosine similarity of the first column vector in the subspace $\textbf{H}^{align}_l$ of each preference, and take the mean across all layers}
\label{tab:preference_pair_correlation}
\end{tabular}
\end{table}

==> tables/urial_exp.tex <==
\begin{table}[t!]
\small
\caption{Compatibility with prompting-based methods.}
   \label{tab:urial_exp}
   \centering
   \begin{tabular}{llcc}
     \toprule
    Model & Dataset & \textbf{$\Delta\%$} \\
    \toprule
     \multirow{3}{*}{Mistral-7B-v0.3} & koala & 9.21 \\
       & oasst & 6.00 \\
       & selfinstruct & 3.54  \\
    
    \midrule

     \multirow{3}{*}{Llama-3.1-8B } & koala & 10.00 \\
       & oasst & 10.00  \\
       & selfinstruct & 5.31  \\
       
      \bottomrule
\end{tabular}
\end{table}
